Cross-Domain Adaptive Teacher for Object Detection

We address the task of domain adaptation in object detection, where there is a domain gap between a domain with annotations (source) and a domain of interest without annotations (target). As an effective semi-supervised learning method, the teacher-student framework (a student model is supervised by the pseudo labels from a teacher model) has also yielded a large accuracy gain in cross-domain object detection. However, it suffers from the domain shift and generates many low-quality pseudo labels (\textit{e.g.,} false positives), which leads to sub-optimal performance. To mitigate this problem, we propose a teacher-student framework named Adaptive Teacher (AT) which leverages domain adversarial learning and weak-strong data augmentation to address the domain gap. Specifically, we employ feature-level adversarial training in the student model, allowing features derived from the source and target domains to share similar distributions. This process ensures the student model produces domain-invariant features. Furthermore, we apply weak-strong augmentation and mutual learning between the teacher model (taking data from the target domain) and the student model (taking data from both domains). This enables the teacher model to learn the knowledge from the student model without being biased to the source domain. We show that AT demonstrates superiority over existing approaches and even Oracle (fully-supervised) models by a large margin. For example, we achieve 50.9% (49.3%) mAP on Foggy Cityscape (Clipart1K), which is 9.2% (5.2%) and 8.2% (11.0%) higher than previous state-of-the-art and Oracle, respectively.

==> exp/city_more.tex <==
\begin{table*}[t]
%   \scriptsize
  \caption{The average precision (AP, in \%) on all classes from different methods for cross-domain object detection on the Foggy Cityscapes test set for \textbf{Cityscapes $\rightarrow$ Foggy Cityscapes} adaptation. The backbone is VGG-16.}

%   \vspace{-2.0mm}
  \centering
  \label{table:videoreid}
  \resizebox{0.85\linewidth}{!}
  {
  \begin{tabular}{lc|cccccccc|c}
  %
  \toprule
  %
  {Method} & Source & bus & bicycle & car & mcycle &person &rider& train &truck& mAP\\
%   \multirow{3}{*}{Method} & \multirow{3}{*}{Source} & \multicolumn{3}{c|}{ConstructSite} & \multicolumn{3}{c|}{WILDTRACK} & \multicolumn{3}{c|}{Mars} & \multicolumn{3}{c}{DukeMTMC}\\
%   %
%   & \multicolumn{4}{c}{Test on: Div-Market}\\
%   \cmidrule{3-14} 
  %
%   \cmidrule{3-14} 
  %
%   & & Rank1 & Rank5 & mAP & Rank1 & Rank5 & mAP & Rank1 & Rank5 & mAP & Rank1 & Rank5 & mAP\\
  %
  \midrule
  Source (F-RCNN)& & 20.1 & 31.86 & 39.64 & 16.93 &  29.03 & 37.17 & 5.17 & 8.14 & 23.5 \\
  Source (F-RCNNfpn)& & 28.41 & 38.61 & 44.9 & 26.16 & 38.94 & 47.43 & 13.46 & 12.51 & 31.3 \\
  \midrule
  SCL~\cite{shen2019scl} & Arxiv19 & 41.8 & 36.2 & 44.8 &33.6& 31.6& 44.0& 40.7& 30.4& 37.9\\
  DA-Faster~\cite{chen2018domain} & CVPR18 & 35.3 &27.1& 40.5& 20.0 &25.0 &31.0 &20.2& 22.1& 27.6\\
  SCDA~\cite{zhu2019adapting} & CVPR19 & 39.0 &33.6 &48.5 &28.0 &33.5 &38.0 &23.3& 26.5& 33.8\\
  SWDA~\cite{saito2019strong} & CVPR19 & 36.2 & 35.3 & 43.5 & 30.0 &  29.9 & 42.3 & 32.6 & 24.5 & 34.3\\
  DM~\cite{kim2019diversify} & CVPR19 & 38.4 &32.2 &44.3 &28.4 &30.8& 40.5 &34.5 & 27.2 & 34.6\\
  MTOR~\cite{cai2019exploring} & CVPR19 & 38.6  &35.6 & 44.0 & 28.3 & 30.6 & 41.4 & 40.6  &21.9 & 35.1\\
  MAF~\cite{he2019multi} & ICCV19 & 39.9 &33.9& 43.9& 29.2 &28.2& 39.5& 33.3& 23.8& 34.0\\
  iFAN~\cite{zhuang2020ifan} & AAAI20 & 45.5& 33.0 &48.5 &22.8 &32.6 &40.0 &31.7& 27.9& 35.3\\
  CRDA~\cite{xu2020exploring} & CVPR20 & 45.1 &34.6& 49.2 &30.3&32.9 &43.8& 36.4 &27.2 &37.4\\
  HTCN~\cite{chen2020harmonizing} & CVPR20 & 47.4 &37.1& 47.9 &32.3& 33.2 &47.5 &40.9 &31.6& 39.8\\
  UMT~\cite{deng2021unbiased} & CVPR21 & 56.5 & 37.3& 48.6 &30.4& 33.0& 46.7 &46.8& 34.1& 41.7\\
  \midrule
  F-RCNN + dis. &  & 37.08 & 41.43 & 54.92 & 31.09 &  38.28 & 46.35 & 16.5 & 22.48 & 36.02\\
%   Baseline (F-RCNN + FPN) \\
  F-RCNNfpn + dis.  &  & 35.83 & 44.76 & 53.34 & 23.55 &  44.58 & 51.58 & 23.14 & 17.44 & 36.78\\
  F-RCNNfpn + pyramid dis.  &  & 36.11 & 45.9 & 53.43 & 29.92 & 46.25 & 53.74 & 11.65 & 19.15 & 37.02\\
  \midrule
  AUT$_\mathrm{base}$ w/o dis & & 58.56 & 53.57 & 63.97 & 38.53 & 45.46 & 55.32 & 43.75 & 33.64 & 49.07\\
  AUT$_\mathrm{base}$ & & 52.82 & 50.09 & 62.88 & 35.33 & 43.93 & 53.77 & 38.01 &30.52& 45.92\\
  AUTfpn$_\mathrm{base}$ w/o dis. & & 64.35 & 57.03 & 73.95 & 45.25 & 60.87 & 64.97 & 52.75 & 35.86 & 56.88 \\
  AUTfpn$_\mathrm{base}$ & & 58.02 &57.57 &71.91 &43.87 & 58.96 & 61.79 & 44.41 &34.22& 53.84 \\
  AUTfpn$_\mathrm{base}$ (pyramid dis.) & & 61.7 & 57.1 & 71.78 & 46.3 & 58.86 & 61.9 &41.46 &34.37 & 54.2\\
  \midrule
%   Ours (UT)  &  & - & - & - & - &  - & - & - & - & 49.12\\
%   Ours (UT + single dis.)  &  & - & - & - & - &  - & - & - & - & 50.09\\
%   Ours (UTfpn)  &  & - & - & - & - &  - & - & - & - & 57.1\\
%   Ours (UTfpn + single dis.)  &  & - & - & - & - &  - & - & - & - & 58.0\\
%   Ours (UTfpn + pyramidal dis.)  &  & - & - & - & - &  - & - & - & - & 58.8\\
%   \midrule
%   Oracle (F-RCNN) &  & - & - & - & - &  - & - & - & - & 42.65 \\
%   Oracle (F-RCNNfpn) &  & - & - & - & - &  - & - & - & - & 52.19
  AUT w/o dis.  &  & 57.49 & 52.63 & 63.84 & 37.45 & 45.51 & 55.28 & 46.75 & 31.81 & 49.26\\
  AUT  &  & 56.3 & 51.87 & 64.17 & 38.47 &  45.53 & 55.05 & 54.34 & 34.99 & 50.85\\
  AUTfpn w/o dis. &  & 65.48 & 58.45 & 74.53 & 46.32 & 60.56 & 64.05& 47.16 & 37.41 & 56.7\\
  AUTfpn  &  & 63.6 & 55.94 & 73.97 & 46.37 & 60.2 & 63.48 & 56.69 & 38.97 & 57.4\\
  AUTfpn (pyramid dis.)  &  & 64.97 & 59.82 & 74.65 & 48.37 & 60.77 & 64.91 & 56.48 & 39.93 & 58.8\\
  \midrule
  Oracle (F-RCNN) &  & 50.28 & 40.72 & 61.28 & 32.46 & 43.06 & 49.74 & 35.11 & 28.56 & 42.65 \\
  Oracle (F-RCNNfpn) &  & 62.37 & 48.19 & 71.05 & 38.26 & 56.65 & 61.07 & 47.21 & 32.74 & 52.19 \\

  \bottomrule
  %
  \end{tabular}
  }
%   \vspace{-3.5mm}
\end{table*}



==> exp/clipart_more.tex <==
\begin{table*}[t]
%   \scriptsize
  \caption{The average precision (AP, in \%) on all classes from different methods for cross-domain object detection on the Clipart1k test set for \textbf{PASCAL VOC $\rightarrow$ Clipart1k} adaptation. The backbone is ResNet-101.}
%   \vspace{-2.0mm}
  \centering
  \label{table:videoreid}
  \resizebox{\linewidth}{!}
  {
  \begin{tabular}{l|cccccccccccccccccccc|c}
  %
  \toprule
  %
  {Method}  & aero & bcycle & bird & boat & bottle &  bus & car & cat &  chair & cow & table & dog & hrs & m-bike & prsn & plnt & sheep &  sofa &  train &  tv & mAP\\
%   \multirow{3}{*}{Method} & \multirow{3}{*}{Source} & \multicolumn{3}{c|}{ConstructSite} & \multicolumn{3}{c|}{WILDTRACK} & \multicolumn{3}{c|}{Mars} & \multicolumn{3}{c}{DukeMTMC}\\
%   %
%   & \multicolumn{4}{c}{Test on: Div-Market}\\
%   \cmidrule{3-14} 
  %
%   \cmidrule{3-14} 
  %
%   & & Rank1 & Rank5 & mAP & Rank1 & Rank5 & mAP & Rank1 & Rank5 & mAP & Rank1 & Rank5 & mAP\\
  %
  \midrule
  Source (F-RCNN) & 23.04 & 39.59 & 20.09 & 23.64 & 25.7 & 42.55 & 25.15 & 0.9 & 41.21 & 25.56 & 23.67 & 11.21 & 28.24 & 49.5 & 45.2 & 46.94 & 9.1 & 22.34 &  38.91 & 31.52 & 28.8\\
  Source (F-RCNNfpn) & 31.82 & 56.38 & 24.6 & 23.29 & 37.56 &  49.29 & 36.69 & 8.55 & 40.98 & 23.12 & 42.25 & 11.3 & 33.77 &  57.37 & 52.97 & 39.6 & 8.2 & 20.28 & 31.1 & 37.8 & 33.1\\
  \midrule
  SCL~\cite{shen2019scl}  & 44.7 & 50.0 & 33.6 & 27.4 & 42.2 & 55.6 & 38.3 & 19.2 & 37.9 & 69.0 & 30.1 & 26.3 & 34.4 &  67.3 & 61.0 & 47.9 & 21.4 & 26.3 & 50.1 & 47.3 & 41.5\\
  SWDA~\cite{saito2019strong}  & 26.2 &48.5 &32.6 &33.7 &38.5& 54.3 &37.1& 18.6& 34.8& 58.3 &17.0 &12.5 &33.8 &65.5 &61.6 &52.0 &9.3 & 24.9 &54.1 &49.1 &38.1\\
  DM~\cite{kim2019diversify} & 25.8 &63.2 &24.5 &42.4 &47.9& 43.1 &37.5 &9.1 &47.0 & 46.7 &26.8& 24.9& 48.1 &78.7& 63.0 &45.0 &21.3& 36.1 &52.3& 53.4 &41.8\\
  CRDA~\cite{xu2020exploring} & 28.7 &55.3 &31.8 &26.0& 40.1& 63.6 &36.6 &9.4 &38.7 & 49.3 &17.6 &14.1 &33.3 &74.3 &61.3 &46.3 &22.3 &24.3 &49.1 &44.3 &38.3\\
  HTCN~\cite{chen2020harmonizing} & 33.6 &58.9 &34.0 &23.4 &45.6 &57.0 &39.8 &12.0 &39.7 & 51.3 &21.1 &20.1 &39.1 &72.8 &63.0 &43.1 &19.3& 30.1& 50.2& 51.8 &40.3\\
  UMT~\cite{deng2021unbiased} & 39.6& 59.1& 32.4 &35.0 &45.1& 61.9&48.4 &7.5 &46.0 & 67.6 &21.4 &29.5 &48.2 &75.9 &70.5 &56.7 &25.9& 28.9 &39.4& 43.6 &44.1\\
  \midrule
  F-RCNN + dis. & 17.4 & 60.96 & 14.81 & 28.0 & 39.25 &  37.11 & 35.88 & 1.6 & 41.84 & 33.41 & 28.74 & 5.72 & 29.64 &  58.34 & 62.71 & 49.19 & 6.74 & 26.69 &  28.04 & 27.29 & 31.6\\
%   Baseline (F-RCNN + FPN) \\
  F-RCNNfpn + dis.  & 24.34 & 50.09 & 27.52 & 25.48 & 45.61 & 44.46 & 29.44 & 6.5 & 49.56 & 47.32 & 40.16 & 6.4 & 29.67 & 58.76 & 57.71 & 56.54 & 25.8 & 16.87 & 32.85 & 37.22 & 35.61\\
  F-RCNNfpn + pyramid dis.   & 17.22 & 53.06 & 24.37 & 27.51 & 49.69 & 49.51 & 30.52 & 14.44 & 50.35 & 39.9 & 44.19 & 11.02 & 23.16 & 58.09 & 46.04 & 47.56 & 23.75 & 29.26 & 35.06 & 35.85 & 34.86\\
  \midrule
  AUT$_\mathrm{base}$ w/o dis & 15.36 & 45.49 & 35.12 & 37.7 & 57.59 & 46.6 & 58.2 & 3.8 & 58.77 & 40.08 & 19.23 & 27.29 & 48.89 & 62.69 & 74.4 &55.26 & 25.73 & 32.74 & 26.62 & 36.07& 40.38\\
  AUT$_\mathrm{base}$ & 24.46 & 54.23 & 31.38 & 41.92 & 57.82 & 72.33 & 49.98 & 3.48 & 55.89 & 54.02 & 34.06 & 23.65& 51.7 & 78.18 &69.84 & 59.23 & 24.79 & 28.15 &40.02 & 41.27 &   45.33\\
  AUTfpn$_\mathrm{base}$ w/o dis. & 42.82 & 45.37 & 30.64 & 43.09 & 61.78 & 62.39 & 54.87 & 7.02 & 57.02 & 45.63 & 42.46 & 17.64 & 38.62 & 84.3 & 73.62 & 66.77 & 19.93 & 37.7 & 49.21 & 57.21 & 46.65\\
  AUTfpn$_\mathrm{base}$ & 34.44 & 59.71 &32.18 & 36.15 & 66.17 & 67.51 & 52.45 & 6.3 & 59.86 & 31.7 & 38.46 & 30.0 & 48.1 & 73.42 & 65.94 & 64.45 & 35.46 &35.54 & 46.19 & 52.77 &46.8\\
  AUTfpn$_\mathrm{base}$ (pyramid dis.)  & 35.19 & 65.14 & 32.43 & 42.75 & 64.59 &  58.67 & 50.92 & 5.3 & 58.14 & 44.84 & 43.0 &  23.55& 45.94 & 77.78 & 67.87 & 58.69  & 31.76 & 38.32 & 46.32& 52.25 & 47.2\\
  \midrule
  AUT w/o dis.  & 15.73 & 39.71 & 30.82 & 41.07 & 57.07 &  46.38 & 50.94 & 4.156 & 60.71 & 28.26 & 34.86 & 29.13 & 51.97 &  58.77 & 73.17 & 58.96 & 21.81 & 32.64 &  28.12 & 46.05 & 40.6\\
  AUT  & 33.82 & 60.85 & 38.57 & 49.41 & 52.36 & 53.92 & 56.69 & 7.467 & 52.83 & 63.52 & 34.04 & 24.95 & 62.24 & 72.05 & 77.15 & 57.67 & 27.2 & 52.04 & 55.65 & 54.12 & 49.3\\
  AUTfpn w/o dis.   & 45.52 & 63.73 & 31.68 & 43.36 & 66.39 & 58.44 & 53.26 & 3.85 & 63.15 & 48.89 & 48.18 & 24.45 & 48.35 & 87.73 & 72.36 & 62.87 & 26.72 & 35.12 & 47.08 & 55.16 & 49.3\\
  AUTfpn   & 39.77 & 65.5 & 34.86 & 42.03 & 63.81 & 65.95 & 54.72 & 6.3 & 62.06 & 45.28 & 44.63 & 27.12 & 53.9 & 89.02 & 73.91 & 65.36 & 29.07 & 28.97 & 45.6 & 54.05 & 51.2\\
  AUTfpn (pyramid dis.)   & 42.53 & 77.66 & 39.33 & 45.0 & 66.57 & 71.07 & 58.27 & 3.59 & 62.53 & 55.36 & 48.16 & 24.08 & 51.56 & 79.16 & 73.85 & 63.11 & 31.11 & 36.62 & 46.96 & 55.29 & 52.5\\
  \midrule
  Oracle (F-RCNN) & 13.23 & 38.75 & 41.54 & 33.23 & 20.92 & 57.88 & 52.81 &22.77 & 42.01 & 23.41 & 36.69 & 32.25 & 29.81 & 44.0 & 69.87 & 42.37 & 45.89 & 17.29 & 52.62 & 45.19 & 38.3\\
   Oracle (F-RCNNfpn) & 22.44 & 35.89 & 40.22 & 40.92 & 28.26 & 49.19 & 61.36 & 18.05 & 45.6 & 53.17 & 45.49 & 31.94 & 34.5 & 66.9 & 74.08 & 46.02 & 49.84 & 23.11 & 54.23 & 53.0 & 43.6\\

  \bottomrule
  %
  \end{tabular}
  }
%   \vspace{-3.5mm}
\end{table*}

% \begin{table*}[t]
% %   \scriptsize
%   \caption{The average precision (AP, in \%) on all classes from different methods for cross-domain object detection on the Clipart1k test set for \textbf{PASCAL VOC $\rightarrow$ Clipart1k} adaptation.}
% %   \vspace{-2.0mm}
%   \centering
%   \label{table:videoreid}
%   \resizebox{\linewidth}{!}
%   {
%   \begin{tabular}{lc|ccccc|c}
%   %
%   \toprule
%   %
%   {Method} & Source & aero & bcycle & bird & boat & bottle & mAP\\
% %   \multirow{3}{*}{Method} & \multirow{3}{*}{Source} & \multicolumn{3}{c|}{ConstructSite} & \multicolumn{3}{c|}{WILDTRACK} & \multicolumn{3}{c|}{Mars} & \multicolumn{3}{c}{DukeMTMC}\\
% %   %
% %   & \multicolumn{4}{c}{Test on: Div-Market}\\
% %   \cmidrule{3-14} 
%   %
% %   \cmidrule{3-14} 
%   %
% %   & & Rank1 & Rank5 & mAP & Rank1 & Rank5 & mAP & Rank1 & Rank5 & mAP & Rank1 & Rank5 & mAP\\
%   %
%   \midrule
%   Source only & & - & - & - & - & - & 27.7\\
%   \midrule
%   SCL~\cite{shen2019scl} & Arxiv19 & 44.7 & 50.0 & 33.6 & 27.4 & 42.2 & 41.5\\
%   SWDA~\cite{saito2019strong} & CVPR19 & 26.2 &48.5 &32.6 &33.7 &38.5&38.1\\
%   DM~\cite{kim2019diversify} & CVPR19 & - & - & - & - & - & 41.8\\
%   CRDA~\cite{xu2020exploring} & CVPR20 & - & - & - & - & - & 38.3\\
%   HTCN~\cite{chen2020harmonizing} & CVPR20 & - & - & - & - & - & 40.3\\
%   UMT~\cite{deng2021unbiased} & CVPR21 & - & - & - & - & - & 44.1\\
%   \midrule
%   Baseline (single dis.) & & - & - & - & - & - & 33.56\\
%   Baseline (pyramidal dis.) & & - & - & - & - & - & 35.35 \\
%   \midrule
% %   Ours (UT) & & - & - & - & - & - & -\\
%   Ours (UT) & & - & - & - & - & - & 49.08 \\
%   Ours (UT + single dis.) & & - & - & - & - & - & 49.98\\
%   Ours (UT + pyramidal dis.) & & - & - & - & - & - & 51.79\\
%   \midrule
%   Oracle & & - & - & - & - & - & 45.0\\

%   \bottomrule
%   %
%   \end{tabular}
%   }
% %   \vspace{-3.5mm}
% \end{table*}

==> experiment_old.tex <==
\section{Experiment}
\label{sec:EXP}

\input{exp/clipart_exp}
\input{exp/city_exp}
% \input{exp/water_exp}
% \input{exp/Ablation_loss}

\subsection{Datasets}
We conduct our experiments on four public datasets, including Cityscapes~\cite{cordts2016cityscapes}, Foggy Cityscapes~\cite{sakaridis2018semantic}, PASCAL VOC~\cite{everingham2010pascal}, and Clipart1k~\cite{inoue2018cross}.

\paragraph{Cityscapes.} Cityscapes~\cite{cordts2016cityscapes} focuses on capturing high variability of outdoor street scenes in common weather conditions from different cities. It contains 2,975 training images and 500 validation images with dense pixel-level labels. We transform the instance segmentation annotations into bounding boxes for our experiments.

\paragraph{Foggy Cityscapes.} Foggy Cityscapes~\cite{sakaridis2018semantic} is built upon the images in the Cityscapes~\cite{cordts2016cityscapes}. This dataset simulates the foggy weather using depth maps provided in Cityscapes with three levels of foggy weather, and thus is suitable to conduct weather adaptation experiments.

\paragraph{PASCAL VOC.} PASCAL VOC~\cite{everingham2010pascal} is a real-world dataset containing 20 categories of common objects with bounding box annotations. Following~\cite{saito2019strong,shen2019scl}, we employ PASCAL VOC 2007 and 2012 training and validation images (16,551 images in total) for experiments.

\paragraph{Clipart1k.} Clipart1k~\cite{inoue2018cross} contains 1k clipart images, which shares the same instance categories with PASCAL VOC but exhibits a large domain shift. We follow the practice in \cite{saito2019strong,shen2019scl}, and use all images of Clipart1k for both training (without labels) and test.

\begin{table}
	\begin{minipage}{0.58\linewidth}
		\caption{The average precision (AP, in \%) on all classes from different methods for cross-domain object detection on the Watercolor2k test set for \textbf{PASCAL VOC $\rightarrow$ Watercolor2k} adaptation. The backbone is ResNet-101.}
		\label{table:student}
		\centering
		\resizebox{\linewidth}{!}
  {
  \begin{tabular}{l|cccccc|c}
  \toprule
  {Method} & bicycle & bird & car & cat & dog & person& mAP\\
  \midrule
  Source (F-RCNN) & 84.2 & 44.5 & 53.0 & 24.9 & 18.8 & 56.3 & 46.9 \\
  \midrule
  SCL~\cite{shen2019scl} & 82.2 & 55.1 & 51.8 & 39.6 & 38.4 & 64.0 & 55.2 \\
  SWDA~\cite{saito2019strong} & 82.3 & 55.9 & 46.5 & 32.7 & 35.5 & 66.7 & 53.3 \\
  UMT~\cite{deng2021unbiased} & 88.2 & 55.3 & 51.7 & 39.8 & 43.6 & 69.9 & 58.1 \\
  \midrule
  AUT (Ours)  & 93.6 & 56.1 & 58.9 & 37.3 & 39.6 & 73.8 & 59.9 \\
  \midrule
  Oracle (F-RCNN) & 51.8 & 49.7 & 42.5 & 38.7 & 52.1 & 68.6 & 50.6 \\
  \bottomrule
  %
  \end{tabular}
  }
	\end{minipage}\hfill
	\begin{minipage}{0.4\linewidth}
		\centering
		\includegraphics[width=\linewidth]{fig/Learning curve.pdf}
		\captionof{figure}{\textbf{Mutual Learning curve on Clipart1k dataset}.}
		\label{fig:curve}
	\end{minipage}
\end{table}
\input{exp/Ablation_loss}
% \begin{figure}[t!]
%   \centering
%   \includegraphics[width=\linewidth]{fig/Learning curve.pdf}
%   \caption{\textbf{Mutual Learning curve on Clipart1k dataset}. Increasing weights of $\lambda_{dis}$ can achieve improved performance and stable learning curve.}
%   \label{fig:curve}
% %   \vspace{-5mm}
% \end{figure}

\subsection{Implementation Details}
Following \cite{chen2018domain,saito2019strong}, we take the Faster RCNN~\cite{ren2015faster} model as the base object detection model in our Adaptive Unbiased Teacher. The ResNet-101~\cite{he2016deep} or VGG16~\cite{simonyan2014very} model pre-trained on ImageNet~\cite{deng2009imagenet} is used as the backbone of the Faster RCNN module. Following the implementation of Faster RCNN with ROI-alignment~\cite{he2017mask}, we rescale all images by setting the shorter side of the image to 600 while keeping the image aspect ratios. For the hyperparameter, we set the $\lambda_{unsup}=1.0$ and $\lambda_{dis}=0.1$ for all the experiments. We set the confidence threshold as $\delta=0.8$. During the initialization stage described in Sec.~\ref{sec:method:mutual}, we train the Faster RCNN using the source labels for 30k iterations. Then we copy the weights to both Teacher and Student models in the beginning of mutual learning and train the adaptive unbiased teacher for 50k iterations. We set the learning rate as 0.04 during the entire training stage without applying any learning rate decay since we found doing so would affect the training efficiency. We optimize the network using Stochastic Gradient Descent (SGD) with weight decay of 0.0005 and momentum of 0.9 For the data augmentation, we apply random horizontal flip for weak augmentation and randomly add color jittering, grayscale, Gaussian blur, and cutout patches for strong augmentations. Note that we do not apply any geometric augmentations. The weight smooth coefficient parameter of the exponential moving average (EMA) for the teacher model is set to 0.9996. Each experiment is conducted on 8 Nvidia GPU V100 with the batch size of 32 and implemented in Pytorch.

\begin{figure*}[t!]
  \centering
  \includegraphics[width=0.95\linewidth]{fig/qual_compare.pdf}
  \caption{\textbf{Qualitative results on Foggy Cityscapes and Clipart1k}. We compare our method with source only and oracle. The first row and the second row are the results of Foggy Cityscapes and Clipart1k, respectively.}
  \label{fig:exp_quali}
%   \vspace{-5mm}
\end{figure*}

\subsection{Experimental Settings and Evaluation}
We report the average precision (AP) of each class as well as the mean AP over all classes for object detection following \cite{chen2018domain,saito2019strong} for all of the experimental settings which are described as follows:
\paragraph{Real to Artistic Adaptation.}
To begin with, we would like to justify the effectiveness of our model for addressing the large domain gap. In this setting, we test our model with domain shift between the real image domain and the artistic image domain. We utilize Pascal VOC as the real source domain and the Clipart1k as the target domain. Clipart1k contains 1k comical images in total, which have the same 20 categories as PASCAL VOC. Following \cite{deng2021unbiased}, the dataset is split equally into a training set and a test set, containing 500 images each. The backbone of ResNet-101~\cite{he2016deep} is used following previous settings.

\paragraph{Weather Adaptation.}
In real-world scenarios, object detectors may be applied under different weather conditions especially for anonymous driving. In this setting, we test our model with domain shift between the image in normal weather and the image with adverse weather (foggy).
The training set of the Cityscapes dataset is used as the source domain while the Foggy Cityscapes dataset is used as the target domain. We take labeled Cityscapes train set images and unlabeled Foggy Cityscapes train set images in our experiment, and report the evaluated results on the validation set of Foggy Cityscapes. Although there exists a one-to-one correspondence between images in Cityscapes and Foggy Cityscapes datasets, we do not leverage such information in unsupervised domain adaptation. The backbone of VGG16~\cite{simonyan2014very} is used following previous settings.




\subsection{Results and Comparisons}
In this section, we report the performance of our adaptive unbiased teacher and other state-of-the-art approaches in Table~\ref{table:cli} and Table~\ref{table:city}. We additionally report the source-only model denoted ``Source (F-RCNN)'' by training a Faster RCNN model using only source images as the lower bound adaptation. On the other hand, we also oracle model denoted ``Oracle (F-RCNN)'' by training a Faster RCNN model using the same images with target domain but with the ground truth annotations, which can be viewed as a reference for the upper bound adaptation performance. 
\paragraph{Real to Artistic Adaptation.}
The results of the setting: real to artistic adaptation is presented in Table~\ref{table:cli}. We compare our method with several state-of-the-art approaches containing  SCL~\cite{shen2019scl}, SWDA~\cite{saito2019strong}, DM~\cite{kim2019diversify}, CRDA~\cite{xu2020exploring}, HTCN~\cite{chen2020harmonizing}, and UMT~\cite{deng2021unbiased}. Some phenomenons can be observed in two folds. First, our model achieves state-of-the-art performance as $49.3\%$ at mAP and outperforms the recent competitor UMT by $5.2\%$ and other methods by a large margin. We note that, UMT using Mean Teacher already has significant performance with augmented-styled training images. However, due to the large domain gap between real and artistic images and incapacity of generating reliable psuedo labels, their model fail to address the bias toward source domain. This demonstrates our model resolves the domain gap with our adaptive unbiased teacher. Second, our model exceeds the oracle model similarly to UMT on this dataset, showing that the mutual learning adopted form Mean Teacher has the potential to bridge the domain gap without utilizing any target labels. The margin around $11\%$ at mAP between our model and the Oracle model can be credited to our efficiency using the source large dataset (PASCAL VOC) when performing the model on the target environment (with only thousands of labels available on Oracle model).


\begin{figure*}[t!]
  \centering
  \includegraphics[width=0.95\linewidth]{fig/abl_qual.pdf}
  \caption{\textbf{Ablation studies of qualitative results on Clipart1k}. This figure show the importance of adversarial loss $\mathcal{L}_{dis}$ and strong augmentation on student model.}
  \label{fig:exp_quali}
%   \vspace{-5mm}
\end{figure*}

% \begin{figure*}[t!]
%   \centering
%   \includegraphics[width=0.95\linewidth]{fig/qual_compare.pdf}
%   \caption{\textbf{Qualitative results on Foggy Cityscapes and Clipart1k}. We compare our method with source only and oracle. The first two rows and the last two row are the results of Foggy Cityscapes and Clipart1k, respectively.}
%   \label{fig:exp_quali}
% %   \vspace{-5mm}
% \end{figure*}

\paragraph{Weather Adaptation.}
The results of the setting: normal weather to adverse weather adaptation is presented in Table~\ref{table:city}. We compare our method with several state-of-the-art approaches containing  SCL~\cite{shen2019scl}, DA-Faster~\cite{chen2018domain}, SCDA~\cite{zhu2019adapting}, MTOR~\cite{cai2019exploring}, MAF~\cite{he2019multi}, iFAN~\cite{zhuang2020ifan}, SWDA~\cite{saito2019strong}, DM~\cite{kim2019diversify}, CRDA~\cite{xu2020exploring}, HTCN~\cite{chen2020harmonizing}, and UMT~\cite{deng2021unbiased}. Some phenomenons can also be observed in this table. First, our model also outperforms all of the state-of-the-art approaches by a large margin (more than 9\%). Among these methods, MTOR~\cite{cai2019exploring} and UMT~\cite{deng2021unbiased} are the two methods adopting Mean Teacher in their model. However, due to the problems discussed earlier regarding the augmentation in Teacher model and bias to source domain, both of their model suffer from generating noisy labels and lead to performance gap between our adaptive unbiased teacher. Second, the performance of our model also exceeds the oracle model by a large margin, showing that the clear weather images with high visibility are useful for boosting the limitation of the object detection in the adverse foggy weather with low visibility, without requiring any annotations on those low visibility images.

\subsection{Ablation studies}
We further conduct ablation studies on the loss functions and the effectiveness of the augmentation pipeline in Table~\ref{table:cli} and Table~\ref{table:city}. The ablation study of loss weight of $\lambda_{dis}$ is also presented in Figure~\ref{fig:curve}.

\paragraph{Adversarial loss $\mathcal{L}_{dis}$}
To further analyze the importance of adversarial learning in our Adaptive Unbiased Teacher, we exclude the loss $\mathcal{L}_{dis}$ in discriminator and report the performance on two experimental settings shown in Table~\ref{table:cli} and Table~\ref{table:city}, respectively. It can be observed that the 9\% performance drop appears in the scenario with larger domain gap (real to artistic adaptation). Yet, in another scenario with smaller domain gap (weather adaptation), only 1.6\% performance drop is observed. 

On the other hand, we also analyze the weight $\lambda_{dis}$ of the adversarial loss $\mathcal{L}_{dis}$ in in Figure~\ref{fig:curve}. Some phenomenons can be observed in this figure in two folds. First, increasing weights can lead to improved performance, which supports the effectiveness of the discriminator in our model. Second, we see that while such hyperparameter $\lambda_{dis}$ need to be determined in advance, the results were not sensitive to their choices (either 0.05 or 0.1). In other words, with a sufficient weight of discriminator loss, the model will be able to have satisfactory performance. Third, the performance with the adversarial loss $\mathcal{L}_{dis}$ shows to be stable without decreasing drastically as the one without the loss.

\paragraph{Augmentation pipeline.}
To justify our design pipeline of augmentation is effectively in our adaptive unbiased teacher, we also conduct the study on it and around 4\% to 5\% performance drop is observed without using our augmentation in both experimental settings, as shown in Table~\ref{table:cli} and Table~\ref{table:city}. This demonstrates that the correct augmentation pipeline (strong and weak augmentation for Teacher and Student, respectively) is vital to our framework.

\paragraph{$\mathcal{L}_{unsup}$ \& EMA.}
To justify the importance of utilizing Mean Teacher and pseudo labels as previous works, we exclude the mutual learning and the Teacher model from our model, and report the performance of the Student model for cross-domain training with only strong augmentation and adversarial loss $\mathcal{L}_{dis}$. We can observe that the performance gain is generally coming from the mutual learning with pseudo labels on target domain. Even with only adversarial loss $\mathcal{L}_{dis}$, our model only improves the source model: Source (F-RCNN) by a small margin on Clipart1k in Table~\ref{table:cli}.


\subsection{Qualitative Analysis}
To further justify the effectiveness of our propose adaptive unbiased teacher (AUT), we present the qualitative results of object detection on the testing set in both settings in Figure~\ref{fig:exp_quali}. We compare our AUT with Source (F-RCNN) model and Oracle (F-RCNN) model. For the setting of weather adaptation, we can observe that there are many missing detections on source model when the fog is serious. Yet, our model is able to achieve the comparable detection result than Oracle model, which demonstrates our model is able to handle domain bias successfully without supervision on target domain. For the setting of real to artistic adaptation, both the Source (F-RCNN) model and Oracle (F-RCNN) model shows missing or incorrect detections in the two given samples. Our AUT instead produce more correct detected bounding boxes than both of the models.



% \input{exp/clipart_exp}
% \input{exp/city_exp}
% \begin{figure*}[t!]
%   \centering
%   \includegraphics[width=\linewidth]{fig/quali.pdf}
%   \caption{\textbf{Qualitative results on Foggy Cityscapes and Clipart1k}. We compare our method with source only and oracle. The first two rows and the third row are the results of Foggy Cityscapes and Clipart1k, respectively.}
%   \label{fig:exp_quali}
% %   \vspace{-5mm}
% \end{figure*}





% \input{exp/clipart_more}
% \input{exp/city_more}



==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

